Diversity of Thought Improves Reasoning Abilities of LLMs

Large language models (LLMs) are documented to struggle in settings that require complex reasoning. Nevertheless, instructing the model to break down the problem into smaller reasoning steps, or ensembling various generations through modifying decoding steps boosts performance. However, these methods assume that the input prompt is fixed and expect the decoding strategies to introduce the diversity needed for ensembling. In this work, we discuss how one can create and leverage variations of the input prompt as a means of diversity of thought. We propose a method that automatically improves prompt diversity by soliciting feedback from the LLM to ideate approaches that are apt for the problem. We then ensemble the diverse prompts in our method DIVSE (DIVerse reasoning path Self-Ensemble) across multiple inference calls, or use diverse approaches within a single inference call; we call the latter IDIV-SE (In-call DIVerse reasoning path Self-Ensemble). Apart from our approaches outperforming prior work, DIV-SE(in particular) advances state-of-the-art performance on the challenging planning and graph coloring benchmarks. Our results improve the Pareto frontier of the accuracy-cost trade-off.

==> gybzwvvpsjbdwnzpcnrrgqyvtmdmnvyb/latex/content/0_abstract.tex <==
\begin{abstract}

Large language models (LLMs) are documented to struggle in settings that require complex reasoning. Nevertheless, instructing the model to break down the problem into smaller reasoning steps, or ensembling various generations through modifying decoding steps boosts performance. However, these methods assume that the input prompt is fixed and expect the decoding strategies to introduce the diversity needed for ensembling.

In this work, we discuss how one can create and leverage variations of the input prompt as a means of \emph{diversity of thought}. 
We propose a method that automatically improves prompt diversity by soliciting feedback from the LLM to ideate approaches that are apt for the problem. We then ensemble the diverse prompts in our method \divse (DIVerse reasoning path Self-Ensemble) across multiple inference calls, or use diverse approaches within a single inference call; we call the latter \idivse (In-call DIVerse reasoning path Self-Ensemble). 
Apart from our approaches outperforming prior work, \textsc{Div-Se} (in particular) advances state-of-the-art performance on the challenging planning and graph  coloring benchmarks. Our results improve the Pareto frontier of the accuracy-cost trade-off.




\end{abstract}  

==> gybzwvvpsjbdwnzpcnrrgqyvtmdmnvyb/latex/content/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}
% P1: Prompting is important, tasks are hard, but techniques are ad-hoc

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{latex/figures/cost_vs_accuracy_besa_feedback.pdf}
    \caption{\textbf{Diversity of Thought enhances the inference cost vs. accuracy trade-off.} We compare DIV-SE and IDIV-SE with SC~\citep{wang2023selfconsistency} and CoT~\citep{wei2022chain} across three benchmarks. The x-axis indicates the total inference cost (as defined in \S~\ref{sec:experiments}) on the benchmark using the given method, while the y-axis represents the LLM’s performance. The few-shot-CoT setting is represented by filled gray dots, while the zero-shot-CoT setting is indicated by unfilled dots. Notice that for a fixed cost, our approaches always give better performance.
}
    \label{fig:cost_vs_accuracy_plot_mert}
\end{figure*}

Large language models (LLMs) exhibit state-of-the-art performance across a myriad of tasks, but their effectiveness is strongly influenced by prompt design~\citep{anil2023palm,openai2023gpt4,nori2023can}. For complex reasoning tasks, the right prompt can enable LLMs to capitalize on task structure~\citep{Guidance:2024:Online}, such as by facilitating memory (by externalizing thought processes), or through tractable problem decomposition~\citep{zhou2024self}. However, existing prompt design either relies on iterative trial-and-error~\citep{white2023prompt}, or is expensive~\citep{lester2021power}.



% P2: 2 general principles that are effective.
Previous works identified two simple, yet general prompting principles to enable complex reasoning: (i) Chain-of-Thought~(CoT) prompting, and (ii) ensembling multiple solutions from diverse decoding paths. CoT prompting~\citep{wei2022chain} improves performance by guiding the LLM to follow step-by-step reasoning. Self-consistency~(SC)~\citep{wang2023selfconsistency} instead increases the stochasticity by modifying the decoding process and obtaining multiple completions, which are then ensembled.

% P3: But combining the two is exxpensive $$$$
However, combining the two principles raises limitations. First, inference is significantly more expensive due to numerous runs, each generating long completions with many reasoning steps. Next, it may be impermissible to modify the decoding process in some settings, such as commercial deployments. Finally, stochasticity-based methods do not directly guide the diversity at the level of thought or method, but rather at the token level. This poses limitations because linguistic token diversity does not always ensure diverse and independent solution approaches.

In this paper, we explore how to explicitly promote the \emph{diversity of thought} while mitigating the aforementioned issues. Prior work by~\citet{li2023making} highlights the importance of prompt diversity, but their notion of diversity is captured through variety in the few-shot examples provided with the prompt; ours focuses on the reasoning approach. We first solicit the LLM to produce multiple-high-level reasoning approaches for problem-solving (e.g., \texttt{method of elimination, visualization techniques} etc. for math reasoning problems). We then leverage GPT-4 to augment few-shot examples used in prior work~\citep{wei2022chain} into the corresponding approaches, whenever applicable. 



% Divse, promotes diversity, gets us better perf.
We propose \divse (DIVerse reasoning path Self-Ensemble) to extract and aggregate responses (via majority vote) across multiple inference calls (\S~\ref{subsec:techniques}). Since distinct approaches introduce diversity at the ``thought'' level, our methodology results in improved ensemble accuracy. In Fig.~\ref{fig:cost_vs_accuracy_plot_mert}, we show that it yields more accurate results across multiple reasoning benchmarks at a fixed inference cost, without modifying the decoding procedure. 
For instance, in the \textsc{Blocksworld 4/5} task~\citep{valmeekam2022large}, \divse improves the performance by 29.6 percentage points (p.p). However, this method still leverages multiple inference calls, which could be costly.

% IDIVse, combining the demos.
To reduce inference costs, we build on the observation that the approaches are often mutually independent, and can be combined in a \emph{single prompt} to solicit multiple solutions~\citep{cheng2023batch}. Based on this premise, we propose \idivse (In-call DIVerse reasoning path Self-Ensemble; \S~\ref{subsec:techniques}), which combines all approaches within the same prompt and aggregates all resulting outputs to leverage diversity with a reduced cost. 
Fig.~\ref{fig:cost_vs_accuracy_plot_mert} demonstrates that this method obtains comparable accuracy to \divse and better performance than prior work with lower inference costs. 

% We push the pareto frontier.
We push the pareto frontier of the cost-accuracy trade-off of prompting strategies across multiple reasoning tasks~(\S~\ref{sec:results}), outperforming both CoT and SC prompting on both GPT-3.5 and GPT-4. This is evident from Fig.~\ref{fig:cost_vs_accuracy_plot_mert} for the \textsc{AQuA-RAT} ~\citep{ling-etal-2017-program}, planning ~\citep{valmeekam2023planning}, and graph coloring~\citep{stechly2023gpt4} benchmarks, where there is a performance improvement of 16.52, 29.6, and 82.5 p.p respectively. These improvements, some of which are state-of-the-art, show the potential of thought diversity to extract complex reasoning abilities from LLMs that were impossible to leverage otherwise. We will open source our code upon publication to encourage further research. 
\input{figures/system_fig}

==> gybzwvvpsjbdwnzpcnrrgqyvtmdmnvyb/latex/content/2_methodology.tex <==

\section{Diversity through LLM Interactions}
\label{sec:method}

First, we introduce terms and notations that we use throughout the paper. We use upper case for sets, lower case for variables, and $[n] = \{1, \cdots, n\}$.

% \begin{itemize}
% \itemsep0em
\noindent{\bf Approach:} These are reasoning strategies for problem solving, denoted with the variable $a$. For example, for the \textsc{GSM8K}~\citep{cobbe2021training}, a benchmark of grade-school math problems
, some of the (generated) approaches can include $a_1=$\texttt{``using visualizations''}, $a_2=$\texttt{``working backwards''}, $a_3=$\texttt{``using direct calculation''}, and $a_4=$\texttt{``method of elimination''}.

\noindent{\bf Persona:} In addition to specifying ``how'' to solve a reasoning problem, specifying a persona can also influence how the LLM behaves~\citep{salewski2023context}. %. 
We denote this with the variable $p$ e.g., $p_1=$\texttt{``Thinking like Alan Turing''}, $p_2=$\texttt{``Thinking like Math Professor''} for the \textsc{GSM8K} task. Note that both approaches and personas are dependent on the reasoning problem. 


\input{latex/content/algorithm}

\subsection{Using the LLM as a guide}
\label{subsec:ap}

Proposed method for creating prompts, which we term {\em \auto} 
 is presented in Algorithm~\ref{alg_1}.
% 
Below, we will describe each step in more detail. At a high-level, we solicit feedback from the LLM on how to solve tasks. 



\noindent{\bf {Step 1+2. Extracting Approaches \& Personas:}} Note that LLMs trained on internet-scale data encode a significant knowledge from multiple domains~\citep{liang2022holistic,bubeck2023sparks}. While LLMs may not be perfect at solving reasoning tasks, we hypothesize that they are helpful in providing high-quality intermediate feedback.

To extract approaches, we utilize the following methodology: (i) Randomly picking a question from the reasoning dataset $D$ we want to evaluate; and (ii) Creating an instruction prompt where we ask the LLM to generate the names of $b \in [1,5]$ {\em approaches} to solve the aforementioned question conforming to a predefined template (for easier post-processing). Refer to Figure~\ref{fig:auto-example} for an example of the prompt used. 

We extract the part of the response that is compliant with the template and store it. We repeat this process $c$ times (obtaining of $c \cdot b$ candidate approaches), and pick the $n$ most frequent approaches to store in set $A$\footnote{\label{note1}In practice, we set $c=100$, $b=5$, $n \in \{3, 5\}$, and $|V| < 20$.}. This process is abstracted as method \texttt{det\_approaches(.)}.

One can repeat the above process used to extract relevant personas for a given reasoning task. However, we followed a simpler route and asked the model directly for relevant personas for a given task and then included them in the set of $m$ candidate personas $P$ used. This is abstracted as method \texttt{det\_personas(.)}. Note that no persona ($\phi$) is also part of the persona set.
%for the final set of prompts. 


\noindent{\bf {Step 3. Choosing the Best Persona, Approach Pairs:}} The choice of persona and approaches introduces a principled way to promote diversity. 
% earlier version
If the set of personas is $P$, and the set of approaches is $A$, the Cartesian product of $P$ and $A$ yields the total number of prompts. In practice, for each combination (denoted by $s_i$) of persona and approach, we evaluate the prompt formed using the composition on a small validation set $V$\textsuperscript{\ref{note1}} and choose the best performing ``\texttt{size}'' elements on the given task\footnote{For a given reasoning task, we perform this process once~(for GPT-3.5 Turbo), and re-use our selection across all LLMs we evaluate. }. 


\noindent{\bf {Step 4. Augmenting few-shot examples:}} Once the (subset of) approach and persona pairs are fixed, we ask the LLM to augment existing few-shot examples %~\mert{What is a demonstration?}
(denoted $F=\{f_1, \cdots\}$) with the given set of approaches. Specifically, we take the few-shot examples provided by~\citet{wei2022chain}, and ask the LLM to solve them in the style of a chosen approach and persona pair (Fig.\ref{fig:algorithm_1_step_4}); we term the output {\em augmented few-shot examples}. This is abstracted in method \texttt{augment(.)}, where $\tilde{T}_{i,j}$ is the set of augmented few-shot examples corresponding to the approach and persona pair from ${s}_i$ and example $f_j$. An example is visualized in the bottom left of Fig.~\ref{fig:overall}, where the prompt contains different approaches for solving a math problem. 

\subsection{Designing the Prompts}
\label{subsec:techniques}

\noindent{\bf Step 5. Prompt Composition:} 
We create prompts for our approach using the best approach and persona pairs identified in step 3, and augmented few-shot examples from step 4 as shown in Fig.~\ref{fig:overall} and~\ref{fig:dev_prompt}.

We now describe two techniques to generate prompts with the augmented demonstrations (${T}$) that have been accumulated.

\vspace{1mm}
\noindent{\bf Candidate 1. \divse:} We first propose \divse (DIVerse reasoning path Self-Ensemble), a method to execute the diverse set of approaches in different inference calls and aggregate their solutions. Apart from the question to be solved and the augmented few-shot examples, the final prompt contains a persona, approach,  and additional instructions. One example is visualized in Fig.~\ref{fig:dev_prompt} (please refer to appendix for more examples of prompts: Fig.~\ref{fig:planning_baseline_prompt} through~\ref{fig:graph_coloring}). {\em Diversity is ensured through running inference with multiple prompts, each with a different approach and persona pairs and augmented few-shot examples.} However, since the approaches are executed separately, generating a solution (via aggregation of multiple responses) requires multiple inference calls, which can be costly. 

\vspace{1mm}
\noindent{\bf Candidate 2. \idivse:} To further reduce the inference costs while promoting diversity, we propose \idivse (In-call DIVerse reasoning path Self-Ensemble). In \idivse, {\em the final prompt is a composition of all approach and persona pairs and corresponding augmented few-shot examples, and the question to be solved}. An example is presented in Fig.~\ref{fig:overall} (bottom left). More examples of prompts are presented in the appendix in Fig.~\ref{fig:planning_baseline_prompt} through~\ref{fig:graph_coloring}. This noticeably decreases the number of calls to be made, since all few-shot examples are presented within the same prompt. We note that there might be error propagation due to the autoregressive nature of models. 
We evaluate this in detail in \S~\ref{error}. 


\noindent{\bf Practicality.} Crucially, \auto finds approaches that are {\em general and reusable} across similar reasoning problems. We reused the strategies identified for solving \textsc{AQuA-RAT} and Planning benchmark respectively in the \textsc{MATH} (counting and probability) and Graph Coloring benchmarks. This also reduces the cost of repeated evaluation on a separate evaluation set.


\noindent{\bf Aggregation.} We aggregate the responses via majority vote for both prompting strategies. Other aggregation strategies can also be leveraged, such as utilizing the LLM itself to aggregate responses or weighted aggregation. In \S~\ref{ss:aggre}, we consider an aggregation strategy proposed by~\citet{yoran2023answering} and describe how compatible it is with our prompting approaches.



==> gybzwvvpsjbdwnzpcnrrgqyvtmdmnvyb/latex/content/3_results.tex <==
%\vspace{-2mm}
\section{Results}
\label{sec:results}
\vspace{-2mm}
\subsection{Main Results}

We present the summary of results in Table~\ref{tab:results_1} and ~\ref{tab:results_2}. Detailed results are available in Appendix~\ref{appendix:addiitonal_results}. These also cover results on the impact of ensemble size in Appendix~\ref{appendix:ensemble_size}.


\begin{table}[t]
\centering
\small
\label{tab:comparison_cqa}
\begin{tabular}{cccc}
\toprule
  {\bf Method} & {\bf Graph Coloring} & {\bf BW 3} & {\bf BW 4/5 } \\
\midrule
 CoT  & 15.0 & 70.00   & 40.00\\
  SC-3 & 18.0 & 66.00   & 38.20\\
  SC-5 & 20.0 & 70.00   & 38.40 \\
  SC-7 & 22.0 &72.00   & 40.00 \\
  SC-10 & 23.0 & 73.00    &41.20 \\
      \idivse & 74.00 & 82.00   & 57.00 \\
      \divse & {\bf 97.00} & {\bf 94.00}  &  {\bf 69.60} \\

\bottomrule
\end{tabular}
\caption{Performance on \textsc{Graph Coloring} and  \textsc{Blocksworld} planning for GPT-4 in the ZS-CoT setting. We compare \divse and
\idivse with SC~\citep{wang2023selfconsistency} and CoT~\citep{wei2022chain}.}
\label{tab:results_1}
\end{table}


\begin{table}[ht]
\centering
\small
\label{tab:comparison_cqa}
\begin{tabular}{ccccccc}
\toprule
{\bf Setting} & {\bf Method} & {\bf AQuA} & {\bf MATH}  & {\bf CQA }\\
\midrule
\multirow{5}{*}{GPT-3.5 ZS} & CoT  & 59.00 & 31.90   &  71.40\\
 & SC-3 & 61.40  & 32.07   &  72.00\\
   & SC-5 & 63.37 & 38.19  &   72.80\\
     & \idivse & 62.60 & 42.50   &  74.00\\
     & \divse & {\bf 72.83} & {\bf 44.94}   & {\bf 74.50} \\ \hline
% & &  &   &  & \\
     \multirow{3}{*}{GPT-3.5 FS} & CoT  & 57.48 & 30.38   &  79.4\\
     & \idivse & 64.57 & 44.10 &  80.00  \\
     & \divse & {\bf 72.84} & {\bf 52.22} &  {\bf 80.40}  \\
\midrule
    \multirow{3}{*}{GPT-4 ZS} &  CoT  & 70.47 & 62.24    & 81.60\\
     & \idivse & 71.65 & 72.00   &  {\bf 82.50 }\\
     & \divse & {\bf 80.31} & {\bf 79.11}    & 81.70\\ \hline
    % & &  &   & & \\
  \multirow{3}{*}{GPT-4 FS}  & CoT  & 71.90 & 66.46  & 87.70\\
     & \idivse & 79.90 & 72.00 &  {\bf 89.00 } \\
     & \divse & {\bf 84.25} & {\bf 80.76}   & 88.00\\
\bottomrule
\end{tabular}
\caption{Performance on \textsc{AQuA-RAT}, \textsc{MATH} (Counting and Probability),  and \textsc{CommonsenseQA} for GPT-3.5 Turbo and GPT-4 in the ZS-CoT and few-shot-CoT settings respectively. \vspace{-5mm} 
}
\label{tab:results_2}
\end{table}

\subsubsection{Arithmetic reasoning via \textsc{AQuA-RAT}} 
\noindent{\em GPT-4 Results:} In Table~\ref{tab:results_2}, we observe that \divse achieves an accuracy increase of 9.84 and 14.6 p.p in the FS-CoT (baseline accuracy of 71.9\%) and ZS-CoT (baseline of 70.47\%) settings, respectively. While the gains from \idivse are nominal in ZS-CoT, it achieves a boost of 7.7 p.p for FS-CoT.

\noindent{\em GPT-3.5 Results:} In Table~\ref{tab:results_2}, we see that \divse yields a gain of 14.23 and 16.52 p.p in the FS-CoT (baseline of 57.48\%) and ZS-CoT (baseline of 59\%) settings, respectively. Within the FS-CoT setting, \idivse gets an absolute increase of 7 p.p.

Note that Fig.~\ref{fig:cost_vs_accuracy_plot_mert} also displays the total inference cost. Both \idivse and \divse are {\em Pareto optimal}, indicating their capacity to achieve a higher accuracy while maintaining low costs.

\subsubsection{Counting and probabilistic reasoning via \textsc{MATH}} 


\noindent{\em GPT-4 Results:} From Table~\ref{tab:results_2}, we see that \divse achieves an accuracy increase of 14.3 and 16.87 p.p in the FS-CoT (baseline of  66.46\%) and ZS-CoT (baseline of 62.24\%) settings, respectively. On the other hand, \idivse achieves a boost of 5.54 and 9.76 p.p in the FS-CoT and ZS-CoT settings, respectively, over the baseline.


\noindent{\em GPT-3.5 Results:} From Table~\ref{tab:results_2}, we see that \divse yields a gain of 21.84 and 13.04 p.p in the FS-CoT (baseline of 30.38\%) and ZS-CoT (baseline of 31.90\%) settings, respectively. Likewise \idivse achieves a boost of 13.72 and 10.60 p.p in the FS-CoT and ZS-CoT settings, respectively.


\subsubsection{Planning via \textsc{Blocksworld}}

 \noindent{\em Setup:} The benchmark provides both natural language and Planning Definition and Domain Language prompts~\citep{mcdermott1998pddl}.
 We use natural language prompts in all the experiments. For the baseline runs, we introduce minor alterations to the prompt originally proposed by~\citet{valmeekam2023planning}. These changes involve incorporating an explicit directive to prevent under-block movement and resolving minor language ambiguities we observed to be problematic during initial investigation. Furthermore, we reposition the initial condition and goal state information to the beginning of the prompt. The modified improved prompt is presented in Fig.~\ref{fig:planning_baseline_prompt}. 
 
We aggregate the plans through majority voting and utilize string matching for comparing the plans. As a result, we optimize the plan by eliminating the redundant ``\texttt{no-op}'' steps.

\begin{comment}
\begin{Verbatim}[commandchars=\\\{\}]
\centering
[(unstack b c), (stack a b), (unstack a b), (stack b a)] ==
[(unstack b c), \sout{(stack a b)}, \sout{(unstack a b)}, (stack b a)] 
\end{Verbatim}
\end{comment}


\noindent{\em GPT-4 Results:} We note that GPT-4 performs slightly better in a ZS setting, and use this to run all experiments. From Fig.~\ref{fig:cost_vs_accuracy_plot_mert}, we observe that for \textsc{Blocksworld 3}, ZS-CoT records an accuracy of 70\%, while SC-10 reaches an accuracy level of 73\%. \idivse enhances the absolute accuracy by 12 p.p above the ZS-CoT baseline, while \divse produces an impressive {\em state-of-the-art} accuracy of 94\%. An analysis of the six unsuccessful instances suggests the capacity for further performance improvement by increasing the size of the ensemble, as already two out of five current approaches generate accurate plans. For the \textsc{Blocksworld 4/5} case, the ZS-CoT accuracy is 40\%, while SC-10 has an accuracy of 41.2\%. Here, \idivse results in an absolute gain of 17 p.p above the ZS-CoT baseline, and \divse too enhances performance, leading to 69.6\%. As outlined in Fig.~\ref{fig:cost_vs_accuracy_plot_mert} and ~\ref{fig:cost_vs_accuracy_plot_mert2}, both \idivse and \divse achieve {\em Pareto optimality}. 

\noindent{\em GPT-3.5 Results:} The baseline performance on \textsc{Blocksworld 3} is 6\%, and on \textsc{Blocksworld 4/5} is 0.6\%. We do not see any additional improvement using both \idivse and \divse. Qualitatively, we observe that during plan generation, GPT-3.5 fails to follow the restrictions provided as part of the problem instructions too often, leading to either infeasible or incorrect plans. This shows instruction following capabilities are crucial to the success of the methods proposed here.

\subsubsection{Constraint Satisfaction via \textsc{graph Coloring}}
There may exist numerous non-optimal yet valid colorings for a given graph. Since exact string matching is not usable for identifying the majority solution from the ensembles of \idivse and \divse, we employ the external, sound verifier~\citep{stechly2023gpt4} to pick the correct solution.

\noindent{\em GPT-4 Results:} From Fig.~\ref{fig:cost_vs_accuracy_plot_mert}, it is observed that ZS-CoT achieves an accuracy of 15\%, whereas SC-10 attains an accuracy level of 23\%. \idivse improves the absolute accuracy by 59 p.p above the ZS-CoT baseline. Remarkably, \divse delivers a {\em state-of-the-art} accuracy of 97\%. Given that GPT-4's performance plateaus in the ZS setting, we  chose to omit conducting the few-shot experiments.


\noindent{\bf Summary:} Methods in this work often demonstrate state-of-the-art performance on reasoning tasks. This is most significant in the planning and constraint satisfaction benchmarks, where the corresponding authors claimed immense difficulty for existing LLMs. Our work shows that status-quo prompt design approaches including chain of thought are too generic for these problems, and prompt customization (via \auto) can yield substantial gains by guiding the chain of thought to the general nature of the problem.



\subsection{Open Source Models}

Due to the limited computational budget, we only performed experiments with the \textsc{AQuA-RAT} benchmark. Please refer to Appendix~\ref{appendix:open-source} for further details. Table~\ref{tab:open-source} demonstrates the results for LLaMA-2 70B with 8-bit quantization. \divse and \idivse demonstrate an improvement of over 10 p.p over the baseline in the FS-CoT settings. However, the gain in the ZS-CoT setting has been negligible. We hypothesize that this is partly due to model's lack of capabilities to both follow instructions and the mentioned approach in the absence of examples. 

\begin{table}[!ht]
  \centering
    \small
  \label{tab:comparison_prompting_strategy}
  \begin{tabular}{lcc}
    \toprule
     {\bf Prompting Strategy} & {\bf ZS-CoT (\%)} & {\bf FS-CoT (\%)} \\
    \midrule
    CoT & 31.32 & 29.1 \\
    \idivse & 27.00 & 39.7 \\
    \divse & \bf{32.00} & \bf{39.9} \\

    \bottomrule
  \end{tabular}
      \caption{Results on \textsc{AQuA-RAT} and LLaMA-2 70B.\vspace{-5mm}}
      \label{tab:open-source}
\end{table}


\subsection{Errors \& Prompt Utility} 
\label{error}


\noindent{\em Error Propagation:} Due to the autoregressive nature of LLM decoding, early incorrect answers in \idivse may get propagated to the latter ones. To quantify this, we select examples where the solution is incorrect and all five approaches produce the same erroneous answer. We focus only on these cases to see if e.g., a wrong conclusion in the initial approaches leaks into the following ones. Next, we attempt the last two approaches again in a separate session: if the LLM generates the same outcomes as in the original session (i.e., \idivse setup) within 3 attempts, we consider it as no error propagation. However, if it does not produce the same answer within the 3 attempts, we interpret this as a case of error propagation since the change in answer could be attributed to the initial approaches with wrong answers in the chain. We measure this phenomenon on \textsc{AQuA-RAT} (FS-CoT) on both GPT-4 and GPT-3.5. We find that GPT-4 and GPT-3.5 have error propagation rates of 6.2\% and 5.5\% respectively, which are comparable to performance differences between \divse and \idivse, {\em making error propagation one of the main explanatory hypotheses for the differences between the two methods}. Reducing these error rates remains a challenging problem given the autoregressive nature of current LLMs. 


\begin{table*}[!ht]
  \centering
\small
  \begin{tabular}{cll}
\toprule
    {\bf Dataset, Model} & {\bf Persona, Approach} & {\bf Accuracy (\%)}  \\
\midrule
    \multirow{3}{*}{\textsc{AQuA-RAT}, GPT-3.5} & $\emptyset$,Think step by step & 57.48  \\
    & $\emptyset$, Using Algebra & 60.24 \footnotesize{\bf (+2.76)} \\
    & Thinking like Alan Turing, $\emptyset$ & 61.81 \footnotesize{\bf (+4.33)}  \\
        & Dr. Patel: A renowned mathematician, $\emptyset$ & {\bf 65.75 \footnotesize{(+8.27)}}  \\
    \hline
    \multirow{3}{*}{\textsc{Blocksworld 4/5}, GPT-4} & $\emptyset$, State tracking prompt~\citep{valmeekam2022large} & 42.00  \\
    & \textcolor{blue}{$\emptyset$, Finite State Machine} & 55.80 \footnotesize{\bf (+13.80)} \\
    & \textcolor{blue}{Alan Turing, Action Rationale} & 57.80 \footnotesize{\bf (+15.80)}  \\
  & \textcolor{blue}{Alan Turing, Progressive Block Placement Approach} & {\bf 58.80 \footnotesize{(+16.80)}}  \\
\bottomrule
  \end{tabular}
    \caption{\textbf{Prompts, derived from approaches and personas, boost performance.} \textcolor{blue}{Blue} rows denote ZS-CoT prompts, while black lines denote FS-CoT prompts. $\emptyset$ denotes absence (of persona or approach respectively). 
    }
 \label{fig:personas_approaches}
\end{table*}

\noindent{\em Beyond Thinking Step by Step:} The diverse approaches and personas we utilize not only enhance the performance in \idivse and \idivse, but are also independently superior to ZS-CoT. Table~\ref{fig:personas_approaches} highlights this effect, which showcases the importance of conditioning the model for solutions via \auto.

\subsection{Alternative Aggregation Strategies}
\label{ss:aggre}

\begin{table}[t]
  \centering
    \small
  \label{tab:comparison_agg_strategy}
  \begin{tabular}{lcc}
    \toprule
     {\bf Method} & {\bf GPT-4 (\%)} & {\bf GPT-3.5 (\%)} \\
    \midrule
    Majority Voting & {\bf 79.90} & 64.47 \\
    Meta Reasoning & {79.24} & {\bf 67.70} \\
    \bottomrule
  \end{tabular}
      \caption{{\bf Alternative aggregation strategies.} Observe that, for the \textsc{AQuA-RAT} benchmark (FS-CoT), \idivse produces more accurate results only with GPT-3.5. \vspace{-5mm}}
      \label{tab:meta}
\end{table}

Our aggregation thus far relies on majority voting. Alternatively, we can also utilize the meta reasoning technique proposed by~\citet{yoran2023answering} to accumulate the results and exploit the rich information present in the reasoning steps.
To this end, we store the responses generated by \idivse, and request the model to meta reason over them in a different prompt and session. Table~\ref{tab:meta} suggests that the proposed reasoning paths contain rich information that is effectively exploited by the meta reasoning aggregation. Future post-hoc  techniques may consider to learn the accuracy of the diverse prompting approaches, and weigh them accordingly. Nevertheless, the fact that techniques presented here provide visible improvements even with simple approaches like majority voting, demonstrates their added value independently from different aggregation algorithms. 



==> gybzwvvpsjbdwnzpcnrrgqyvtmdmnvyb/latex/content/4_related_work.tex <==
\section{Related Work}
\label{sec:related}
\noindent{\bf Prompt Optimization:} \citet{pryzant2023automatic} models the prompts as optimizable discrete variables, and minimizes the loss of the reasoning task. \citet{jones2023automatically} optimize over the prompt space, but to identify failure modes. However, optimization-based approaches often require the task to have a differentiable loss function, which is a strong condition. In our work, we utilize feedback from the LLM (not through gradients) during prompt design. Similarly to~\citet{cheng2023batch}, \idivse batches the responses for multiple queries within a prompt.

\noindent{\bf Decoding Optimizations and Tools:}~\citet{wang2023selfconsistency} replace the naive greedy decoding by sampling a diverse set of reasoning paths (e.g., through temperature sampling), and then selects the most consistent answer. ~\citet{chen2022program} express the reasoning process as a program, which is then delegated to an external tool. 
In our work, we neither change the decoding process nor assume the existence of trusted tools. This makes our solution directly applicable to black-box models.

\noindent{\bf Prompting Strategies:} ~\citet{brown2020language} note that demonstrations to prompts, encoded as input-output pairs, produce drastic performance increase in larger LLMs.~\citet{wei2022chain} encourage internal dialogue by forcing the LLM to generate a sequence of intermediate steps for reasoning problems. This improves reasoning performance on larger LLMs~\citep{nye2021show,chung2022scaling, kojima2022large}. ~\citet{zhou2022least} automatically break a complex problem into simpler sub-problems and then solve them in sequence. Across all these techniques, the common practice is to keep the prompts fixed, but aggregate responses across multiple trials by varying the temperature. In our work, we vary the input prompt itself. A work that is similar in spirit is that of~\citet{yoran2023answering}, which instead of aggregating the response of multiple reasoning paths, forces the model to reason across them before aggregation. Another relevant work is that of \citet{li2023making}, which shows the importance of prompt diversity. However, they rely on selecting few-shot demonstrations from a hold-out set (which defines diversity in their method), without explicitly stating reasoning pathways. 



==> gybzwvvpsjbdwnzpcnrrgqyvtmdmnvyb/latex/content/5_conclusions.tex <==
\section{Conclusions}
In this work, we promoted diversity of thought as a principled prompting strategy and proposed methodologies that leverage the LLM as a guide to design a diverse set of approaches to solve complex reasoning tasks. Extracting solution approaches from LLMs themselves becomes a discovery mechanism that seeds and conditions generative solutions. 
Reported results on a variety of tasks confirm that there is a large space for improvement in complex reasoning by uncovering the necessary skills and knowledge from LLMs through targeted and diverse prompting methods. These results demonstrated how promoting diversity can improve the Pareto frontier of accuracy-cost trade-off for current LLMs and yield {\em state-of-the-art} solutions for planning and mathematical reasoning tasks. We hope that future work will expand these results to complex tasks from other real-world applications. 


\section{Limitations}
Our study mainly experimented with GPT-3.5 and GPT-4 models because of their instruction-following capabilities. While current open-source models have shown remarkable improvements to this end, they are still not able to reliably follow instructions relevant to complex reasoning tasks (e.g. state tracking, plan validity, constraint satisfaction). We hope that progress in the field will enable further experimentation in this direction. 

In addition, we also observe that error propagation during autoregressive generation may sometimes negatively impact the performance of \idivse, where all approaches are executed in order within the same prompt. Some of this could be addressed by explicitly instructing the model to forget about the previous solution but ultimately as long as previous generation history remains in context and short-term memory, error propagation risks may still need to be tracked and measured. 






==> gybzwvvpsjbdwnzpcnrrgqyvtmdmnvyb/latex/content/algorithm.tex <==

\begin{algorithm}[t]
\footnotesize
\captionsetup{labelformat=empty}
\caption{{\em \auto}: Prompt creation.}
\begin{algorithmic}
\Procedure{DiversePrompt}{\texttt{size, type}, $F, D, V$}
\State \LeftComment \textbf{Step 1: Identify different approaches to be used.}
\State $A = \{a_1, \ldots, a_{n}\} \gets \texttt{det\_approaches}(\texttt{D})$ 
\LeftComment{where $A$ is the set of approaches}
\State \LeftComment \textbf{Step 2: Identify different personas to be used.}
\State $P = \{\phi, p_1, \ldots, p_{m}\} \gets \texttt{det\_personas}(\texttt{D})$ 
\LeftComment{where $P$ is the set of personas}
\State \LeftComment \textbf{Step 3: Find the best combination.}
%of approaches and personas.}
\State $ S = \{s_1, \ldots\, s_{\texttt{size}}\} \gets \texttt{combine}(A, P, \texttt{size}, V)$ 
\LeftComment{where $S$ is the set of combined approaches and personas, and $s_i = (p, a_{i} \in A)$}
\State \LeftComment \textbf{Step 4: Augment the few-shot examples.}
%\State $T = \{f((p_i, a_j), FS), f((p_i, a_k),_FS),\ldots\} \gets \texttt{transfer}(S, F)$ \LeftComment{where $T$ is the set of style-transferred examples}
\State $T = \{\tilde{T}_{i,j}, \ldots\} \gets \texttt{augment}(S, F)$ \LeftComment{where $T$ is the set of augmented examples, and $\tilde{T}_{i,j}$ is formed using $s_i \in S$ and $f_j \in F$; $|T|=$\texttt{size}}
\State \LeftComment \textbf{Step 5: Compose the final prompt.}
%based on $T$, $S$, and \texttt{type}.}
\State $O \gets \texttt{compose}(T, S, \texttt{type})$ 
\State \textbf{return } $O$ \LeftComment{Return the final output.}
\EndProcedure
\end{algorithmic}
\label{alg_1}
\end{algorithm}






==> gybzwvvpsjbdwnzpcnrrgqyvtmdmnvyb/latex/content/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
%\noindent{\bf Tasks \& Datasets.} 
We consider the following reasoning benchmarks.
%\begin{enumerate}[leftmargin=*,itemsep=0.0ex, parsep=0pt] 

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{latex/figures/cost_vs_accuracy_gsm_cqa_besa_feedback.pdf}
    \caption{\textbf{Diversity of Thought enhances the inference cost and accuracy trade-off.} We compare \divse and \idivse with SC~\citep{wang2023selfconsistency} and CoT~\citep{wei2022chain} across three benchmarks. The x-axis indicates the total cost (as defined in \S~\ref{sec:experiments}) of running inference with the LLM on the benchmark using the given method, while the y-axis represents the LLM’s performance. The FS-CoT setting is represented by filled gray dots, while the ZS-CoT setting is indicated by unfilled dots. Notice that for \textsc{Blocksworld 3}, despite being in the ZS-CoT setting, our approaches are more performant than the SC-$s$ (FS-CoT) baseline.\vspace{-5mm}}
    \label{fig:cost_vs_accuracy_plot_mert2}
\end{figure*}


\noindent {\em Arithmetic Reasoning}:  We use: (i) \textsc{AQuA-RAT}~\citep{ling-etal-2017-program}, a suite of algebraic word problems,  (ii) \textsc{GSM8K}~\citep{cobbe2021training}, a benchmark of grade-school math problems described in natural language (involving elementary arithmetic operations), and (iii) \textsc{MATH} (Counting and Probability)~\citep{hendrycks2021measuring}, a collection of math problems from which we choose only counting and probability as these are not covered by \textsc{GSM8K} and \textsc{AQuA-RAT}. For all datasets, we use the \texttt{test} split for evaluation, containing 254, 1319, and 474 questions respectively. 

\noindent {\em Planning Capabilities}: We use the Blocksworld Planning benchmark proposed in \citet{valmeekam2022large, valmeekam2023planning}. 
The benchmark has two datasets: one involves 3 blocks (\textsc{Blocksworld 3}, 100 instances), while the other dataset involves 4 or 5 blocks (\textsc{Blocksworld 4/5}, 500 instances). 

\noindent {\em Constraint Satisfaction Optimization}: We use the \textsc{Graph coloring} benchmark~\citep{stechly2023gpt4} containing 100 examples to test reasoning for constraint satisfaction.

\noindent {\em Commonsense Reasoning}: We use \textsc{CommonsenseQA}~\citep{talmor-etal-2019-commonsenseqa} which consists of generic multiple-choice questions elicited for testing common sense reasoning. We use the \texttt{validation} split containing 1,221 questions.


\noindent{\bf Language Models.} We evaluate our proposed methods on both GPT-3.5 Turbo~\citep{chatgpt} and GPT-4~\citep{gpt4}. We also conduct an additional evaluation on LLaMA-2 70B~\citep{touvron2023llama2} to explore the performance of our technique on open-source LLMs. For the latter, we use \texttt{meta-llama/Llama-2-70b-chat-hf} through the Transformers library~\citep{wolf2019huggingface}.



\noindent{\bf Baselines.} We consider Chain-of-Thought (CoT)~\citep{wei2022chain} and Self-Consistency (SC~)~\citep{wang2023selfconsistency} as our baselines. For CoT, we consider two settings: zero-shot (ZS) CoT~\citep{kojima2022large} (i.e., ``\texttt{Think step by step}'' is added to the prompt), and few-shot (FS) CoT (i.e., CoT with demonstrations). In our SC runs, we set the temperature $T=0.7$ without top-$k$ truncation and sample up to $s \in [1,10]$ outputs (denoted SC-$s$). For all other approaches, we set $T=0$. We use ensembles of size 5 in \idivse and  \divse for \textsc{GSM8K} and \textsc{AQuA-RAT}. For the planning, \textsc{Graph Coloring}, and \textsc{CommonsenseQA} benchmarks, we use a size of 3. 

%\iffalse
\noindent{\bf Performance Metrics.} We measure the accuracy on the task, and the generation inference cost.To measure the cost, we assume 1000 tokens are about 750 words\footnote{https://openai.com/pricing}. For GPT-4 (8K) the input and output prices used to estimate inference cost are \$0.03/1k tokens and \$0.06/1k tokens, respectively. For GPT 3.5 Turbo (16K), the input and output prices used in the cost estimation are \$0.003/1k (tokens) and \$0.004/1k (tokens) respectively. 
%\fi

\noindent{\bf Results Summary.} %Salient features of our results include:
\noindent 
\noindent Across most benchmarks we consider, our techniques provide substantial performance gains (e.g., 16.52, 82.5, and 14.3 p.p improvements for \textsc{AQuA-RAT}, \textsc{Graph Coloring}, and \textsc{MATH} respectively). They are also Pareto optimal (in terms of the utility vs. cost trade-off). For the challenging planning benchmark (\textsc{Blocksworld 4/5}), our techniques improve accuracy by 29.6 p.p achieving {\em state-of-the-art} performance. Using GPT-4 for \textsc{Blocksworld 3}, our approach (in the ZS-CoT setting) is substantially more effective than SC-10 (in the FS-CoT setting) at 4$\times$ lower cost (Figure~\ref{fig:cost_vs_accuracy_plot_mert2} (center figure)). 

Since prompts are chained together in \idivse, error propagation is possible. Our evaluation on \textsc{AQuA-RAT} in ~\S~\ref{error} suggests that even though error propagation is estimated as less than 6.5\% for both models, these rates are comparable to differences in performance between \divse and \idivse. 
\noindent When combined with aggregation approaches that are capable of reasoning across the diverse generations~\citep{yoran2023answering}, we observe additional performance gains as shown in ~\S~\ref{ss:aggre}. For the \textsc{AQuA-RAT} benchmark for instance, we see an accuracy of 67.7\% for GPT-3.5 (3.23 p.p improvement to majority voting). 
%\end{enumerate}

==> gybzwvvpsjbdwnzpcnrrgqyvtmdmnvyb/latex/figures/intro_fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{latex/figures/cost_vs_accuracy_v2.pdf}
    \caption{\textbf{Diversity of Thought enhances the inference cost and accuracy trade-off.} We compare \divse and \idivse with SC~\citep{wang2023selfconsistency} and CoT~\citep{wei2022chain} across three benchmarks. Panels show (i) AQUA-RAT on GPT-3.5 in few-shot-CoT setting, and (ii) Blocksworld 3 and 4/5 on GPT-4 in zero-shot-CoT setting. The x-axis indicates the total cost (as defined in \S~\ref{sec:results}) of running inference with the LLM on the benchmark with the given approach, the y-axis indicates the LLM's performance, and the color indicates the approach (and whether it is zero-shot-CoT or few-shot-CoT).}
    \label{fig:cost_vs_accuracy_plot_mert}
\end{figure}




==> gybzwvvpsjbdwnzpcnrrgqyvtmdmnvyb/latex/figures/prompt_example.tex <==
\definecolor{lightgray}{RGB}{240,240,240} %
\renewcommand{\sfdefault}{cmss} % Computer Modern Sans Serif
\begin{figure*}[!th]
\begin{tcolorbox}[
    enhanced,
    opacityback=0.2,
    opacityframe=0.2,
    colback=lightgray,
    colframe=lightgray, 
    top=1mm, 
    bottom=1mm, 
    left=1mm, 
    right=1mm,
    %sharp corners,
    fontupper=\sffamily\small,
    ]    
\begin{small}
\noindent

Use five distinct approaches to solve the given problem accurately. If there is no exact match choose the closest option.

Q: \{Question\}

Use the following output format:

Approach 1 {< name of the approach >} : {< Details of Approach 1} >

Approach 2 {< name of the approach >} : {< Details of Approach 2} >

Approach 3 {< name of the approach >} : {< Details of Approach 3} >

Approach 4 {< name of the approach >} : {< Details of Approach 4} >

Approach 5 {< name of the approach >} : {< Details of Approach 5} >
\noindent
\end{small}
\end{tcolorbox}
\caption{Prompt template for extracting diverse approaches for problem solving.}
\label{fig:auto-example}
\end{figure*}

\clearpage

==> gybzwvvpsjbdwnzpcnrrgqyvtmdmnvyb/latex/figures/system_fig.tex <==
\begin{figure*}[t]
\centering
\begin{minipage}[t]{0.9\textwidth}
\includegraphics[width=\linewidth]{figures/system_diagram_1_3.pdf}
\end{minipage}
\caption{\textbf{Diversity of Thought}. This illustration depicts CoT and \idivse prompting strategies. Notice that both have a single example. However, \idivse presents more diversity in terms of reasoning paths. This enables it to generate diverse completions, yielding more accurate responses.\vspace{-5mm}}
\label{fig:overall}
\end{figure*}



==> latex/figures/intro_fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{latex/figures/cost_vs_accuracy_v2.pdf}
    \caption{\textbf{Diversity of Thought enhances the inference cost and accuracy trade-off.} We compare \divse and \idivse with SC~\citep{wang2023selfconsistency} and CoT~\citep{wei2022chain} across three benchmarks. Panels show (i) AQUA-RAT on GPT-3.5 in few-shot-CoT setting, and (ii) Blocksworld 3 and 4/5 on GPT-4 in zero-shot-CoT setting. The x-axis indicates the total cost (as defined in \S~\ref{sec:results}) of running inference with the LLM on the benchmark with the given approach, the y-axis indicates the LLM's performance, and the color indicates the approach (and whether it is zero-shot-CoT or few-shot-CoT).}
    \label{fig:cost_vs_accuracy_plot_mert}
\end{figure}




==> latex/macros.tex <==
\newif\ifdraft

\drafttrue
% \draftfalse

\ifdraft
\newcommand{\varun}[1]{\textcolor{red}{VC:#1}}
\newcommand{\ranjita}[1]{\textcolor{cyan}{RN:#1}}
\newcommand{\besa}[1]{\textcolor{orange}{BN:#1}}
\newcommand{\mert}[1]{\textcolor{blue}{MY:#1}}

\else
\newcommand{\varun}[1]{}
\newcommand{\ranjita}[1]{}
\newcommand{\besa}[1]{}
\newcommand{\mert}[1]{}

\fi



==> macros.tex <==
\newif\ifdraft

\drafttrue
% \draftfalse

\ifdraft
\newcommand{\varun}[1]{\textcolor{red}{VC:#1}}
\newcommand{\ranjita}[1]{\textcolor{cyan}{RN:#1}}
\newcommand{\besa}[1]{\textcolor{orange}{BN:#1}}
\newcommand{\mert}[1]{\textcolor{blue}{MY:#1}}

\else
\newcommand{\varun}[1]{}
\newcommand{\ranjita}[1]{}
\newcommand{\besa}[1]{}
\newcommand{\mert}[1]{}

\fi



==> xkzmfysyngmvcnyzvsrzkvmqbwygckny/latex/content/0_abstract.tex <==
\begin{abstract}

Large language models (LLMs) are documented to struggle in settings that require complex reasoning. Nevertheless, instructing the model to break down the problem into smaller reasoning steps, or ensembling various generations through modifying decoding steps boosts performance. However, these methods assume that the input prompt is fixed and expect the decoding strategies to introduce the diversity needed for ensembling.

In this work, we discuss how one can create and leverage variations of the input prompt as a means of \emph{diversity of thought}. 
We propose a method that automatically improves prompt diversity by soliciting feedback from the LLM to ideate approaches that are apt for the problem. We then ensemble the diverse prompts in our method \divse (DIVerse reasoning path Self-Ensemble) across multiple inference calls, or use diverse approaches within a single inference call; we call the latter \idivse (In-call DIVerse reasoning path Self-Ensemble). 
Apart from our approaches outperforming prior work, \textsc{Div-Se} (in particular) advances state-of-the-art performance on the challenging planning and graph  coloring benchmarks. Our results improve the Pareto frontier of the accuracy-cost trade-off.




\end{abstract}  

==> xkzmfysyngmvcnyzvsrzkvmqbwygckny/latex/content/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}
% P1: Prompting is important, tasks are hard, but techniques are ad-hoc

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{latex/figures/cost_vs_accuracy_besa_feedback.pdf}
    \caption{\textbf{Diversity of Thought enhances the inference cost vs. accuracy trade-off.} We compare DIV-SE and IDIV-SE with SC~\citep{wang2023selfconsistency} and CoT~\citep{wei2022chain} across three benchmarks. The x-axis indicates the total inference cost (as defined in \S~\ref{sec:experiments}) on the benchmark using the given method, while the y-axis represents the LLM’s performance. The few-shot-CoT setting is represented by filled gray dots, while the zero-shot-CoT setting is indicated by unfilled dots. Notice that for a fixed cost, our approaches always give better performance.
}
    \label{fig:cost_vs_accuracy_plot_mert}
\end{figure*}

Large language models (LLMs) exhibit state-of-the-art performance across a myriad of tasks, but their effectiveness is strongly influenced by prompt design~\citep{anil2023palm,openai2023gpt4,nori2023can}. For complex reasoning tasks, the right prompt can enable LLMs to capitalize on task structure~\citep{Guidance:2024:Online}, such as by facilitating memory (by externalizing thought processes), or through tractable problem decomposition~\citep{zhou2024self}. However, existing prompt design either relies on iterative trial-and-error~\citep{white2023prompt}, or is expensive~\citep{lester2021power}.



% P2: 2 general principles that are effective.
Previous works identified two simple, yet general prompting principles to enable complex reasoning: (i) Chain-of-Thought~(CoT) prompting, and (ii) ensembling multiple solutions from diverse decoding paths. CoT prompting~\citep{wei2022chain} improves performance by guiding the LLM to follow step-by-step reasoning. Self-consistency~(SC)~\citep{wang2023selfconsistency} instead increases the stochasticity by modifying the decoding process and obtaining multiple completions, which are then ensembled.

% P3: But combining the two is exxpensive $$$$
However, combining the two principles raises limitations. First, inference is significantly more expensive due to numerous runs, each generating long completions with many reasoning steps. Next, it may be impermissible to modify the decoding process in some settings, such as commercial deployments. Finally, stochasticity-based methods do not directly guide the diversity at the level of thought or method, but rather at the token level. This poses limitations because linguistic token diversity does not always ensure diverse and independent solution approaches.

In this paper, we explore how to explicitly promote the \emph{diversity of thought} while mitigating the aforementioned issues. Prior work by~\citet{li2023making} highlights the importance of prompt diversity, but their notion of diversity is captured through variety in the few-shot examples provided with the prompt; ours focuses on the reasoning approach. We first solicit the LLM to produce multiple-high-level reasoning approaches for problem-solving (e.g., \texttt{method of elimination, visualization techniques} etc. for math reasoning problems). We then leverage GPT-4 to augment few-shot examples used in prior work~\citep{wei2022chain} into the corresponding approaches, whenever applicable. 



% Divse, promotes diversity, gets us better perf.
We propose \divse (DIVerse reasoning path Self-Ensemble) to extract and aggregate responses (via majority vote) across multiple inference calls (\S~\ref{subsec:techniques}). Since distinct approaches introduce diversity at the ``thought'' level, our methodology results in improved ensemble accuracy. In Fig.~\ref{fig:cost_vs_accuracy_plot_mert}, we show that it yields more accurate results across multiple reasoning benchmarks at a fixed inference cost, without modifying the decoding procedure. 
For instance, in the \textsc{Blocksworld 4/5} task~\citep{valmeekam2022large}, \divse improves the performance by 29.6 percentage points (p.p). However, this method still leverages multiple inference calls, which could be costly.

% IDIVse, combining the demos.
To reduce inference costs, we build on the observation that the approaches are often mutually independent, and can be combined in a \emph{single prompt} to solicit multiple solutions~\citep{cheng2023batch}. Based on this premise, we propose \idivse (In-call DIVerse reasoning path Self-Ensemble; \S~\ref{subsec:techniques}), which combines all approaches within the same prompt and aggregates all resulting outputs to leverage diversity with a reduced cost. 
Fig.~\ref{fig:cost_vs_accuracy_plot_mert} demonstrates that this method obtains comparable accuracy to \divse and better performance than prior work with lower inference costs. 

% We push the pareto frontier.
We push the pareto frontier of the cost-accuracy trade-off of prompting strategies across multiple reasoning tasks~(\S~\ref{sec:results}), outperforming both CoT and SC prompting on both GPT-3.5 and GPT-4. This is evident from Fig.~\ref{fig:cost_vs_accuracy_plot_mert} for the \textsc{AQuA-RAT} ~\citep{ling-etal-2017-program}, planning ~\citep{valmeekam2023planning}, and graph coloring~\citep{stechly2023gpt4} benchmarks, where there is a performance improvement of 16.52, 29.6, and 82.5 p.p respectively. These improvements, some of which are state-of-the-art, show the potential of thought diversity to extract complex reasoning abilities from LLMs that were impossible to leverage otherwise. We will open source our code upon publication to encourage further research. 
\input{latex/figures/system_fig}

==> xkzmfysyngmvcnyzvsrzkvmqbwygckny/latex/content/2_methodology.tex <==

\section{Diversity through LLM Interactions}
\label{sec:method}

First, we introduce terms and notations that we use throughout the paper. We use upper case for sets, lower case for variables, and $[n] = \{1, \cdots, n\}$.

% \begin{itemize}
% \itemsep0em
\noindent{\bf Approach:} These are reasoning strategies for problem solving, denoted with the variable $a$. For example, for the \textsc{GSM8K}~\citep{cobbe2021training}, a benchmark of grade-school math problems
, some of the (generated) approaches can include $a_1=$\texttt{``using visualizations''}, $a_2=$\texttt{``working backwards''}, $a_3=$\texttt{``using direct calculation''}, and $a_4=$\texttt{``method of elimination''}.

\noindent{\bf Persona:} In addition to specifying ``how'' to solve a reasoning problem, specifying a persona can also influence how the LLM behaves~\citep{salewski2023context}. %. 
We denote this with the variable $p$ e.g., $p_1=$\texttt{``Thinking like Alan Turing''}, $p_2=$\texttt{``Thinking like Math Professor''} for the \textsc{GSM8K} task. Note that both approaches and personas are dependent on the reasoning problem. 


\input{latex/content/algorithm}

\subsection{Using the LLM as a guide}
\label{subsec:ap}

Proposed method for creating prompts, which we term {\em \auto} 
 is presented in Algorithm~\ref{alg_1}.
% 
Below, we will describe each step in more detail. At a high-level, we solicit feedback from the LLM on how to solve tasks. 



\noindent{\bf {Step 1+2. Extracting Approaches \& Personas:}} Note that LLMs trained on internet-scale data encode a significant knowledge from multiple domains~\citep{liang2022holistic,bubeck2023sparks}. While LLMs may not be perfect at solving reasoning tasks, we hypothesize that they are helpful in providing high-quality intermediate feedback.

To extract approaches, we utilize the following methodology: (i) Randomly picking a question from the reasoning dataset $D$ we want to evaluate; and (ii) Creating an instruction prompt where we ask the LLM to generate the names of $b \in [1,5]$ {\em approaches} to solve the aforementioned question conforming to a predefined template (for easier post-processing). Refer to Figure~\ref{fig:auto-example} for an example of the prompt used. 

We extract the part of the response that is compliant with the template and store it. We repeat this process $c$ times (obtaining of $c \cdot b$ candidate approaches), and pick the $n$ most frequent approaches to store in set $A$\footnote{\label{note1}In practice, we set $c=100$, $b=5$, $n \in \{3, 5\}$, and $|V| < 20$.}. This process is abstracted as method \texttt{det\_approaches(.)}.

One can repeat the above process used to extract relevant personas for a given reasoning task. However, we followed a simpler route and asked the model directly for relevant personas for a given task and then included them in the set of $m$ candidate personas $P$ used. This is abstracted as method \texttt{det\_personas(.)}. Note that no persona ($\phi$) is also part of the persona set.
%for the final set of prompts. 


\noindent{\bf {Step 3. Choosing the Best Persona, Approach Pairs:}} The choice of persona and approaches introduces a principled way to promote diversity. 
% earlier version
If the set of personas is $P$, and the set of approaches is $A$, the Cartesian product of $P$ and $A$ yields the total number of prompts. In practice, for each combination (denoted by $s_i$) of persona and approach, we evaluate the prompt formed using the composition on a small validation set $V$\textsuperscript{\ref{note1}} and choose the best performing ``\texttt{size}'' elements on the given task\footnote{For a given reasoning task, we perform this process once~(for GPT-3.5 Turbo), and re-use our selection across all LLMs we evaluate. }. 


\noindent{\bf {Step 4. Augmenting few-shot examples:}} Once the (subset of) approach and persona pairs are fixed, we ask the LLM to augment existing few-shot examples %~\mert{What is a demonstration?}
(denoted $F=\{f_1, \cdots\}$) with the given set of approaches. Specifically, we take the few-shot examples provided by~\citet{wei2022chain}, and ask the LLM to solve them in the style of a chosen approach and persona pair (Fig.\ref{fig:algorithm_1_step_4}); we term the output {\em augmented few-shot examples}. This is abstracted in method \texttt{augment(.)}, where $\tilde{T}_{i,j}$ is the set of augmented few-shot examples corresponding to the approach and persona pair from ${s}_i$ and example $f_j$. An example is visualized in the bottom left of Fig.~\ref{fig:overall}, where the prompt contains different approaches for solving a math problem. 

\subsection{Designing the Prompts}
\label{subsec:techniques}

\noindent{\bf Step 5. Prompt Composition:} 
We create prompts for our approach using the best approach and persona pairs identified in step 3, and augmented few-shot examples from step 4 as shown in Fig.~\ref{fig:overall} and~\ref{fig:dev_prompt}.

We now describe two techniques to generate prompts with the augmented demonstrations (${T}$) that have been accumulated.

\vspace{1mm}
\noindent{\bf Candidate 1. \divse:} We first propose \divse (DIVerse reasoning path Self-Ensemble), a method to execute the diverse set of approaches in different inference calls and aggregate their solutions. Apart from the question to be solved and the augmented few-shot examples, the final prompt contains a persona, approach,  and additional instructions. One example is visualized in Fig.~\ref{fig:dev_prompt} (please refer to appendix for more examples of prompts: Fig.~\ref{fig:planning_baseline_prompt} through~\ref{fig:graph_coloring}). {\em Diversity is ensured through running inference with multiple prompts, each with a different approach and persona pairs and augmented few-shot examples.} However, since the approaches are executed separately, generating a solution (via aggregation of multiple responses) requires multiple inference calls, which can be costly. 

\vspace{1mm}
\noindent{\bf Candidate 2. \idivse:} To further reduce the inference costs while promoting diversity, we propose \idivse (In-call DIVerse reasoning path Self-Ensemble). In \idivse, {\em the final prompt is a composition of all approach and persona pairs and corresponding augmented few-shot examples, and the question to be solved}. An example is presented in Fig.~\ref{fig:overall} (bottom left). More examples of prompts are presented in the appendix in Fig.~\ref{fig:planning_baseline_prompt} through~\ref{fig:graph_coloring}. This noticeably decreases the number of calls to be made, since all few-shot examples are presented within the same prompt. We note that there might be error propagation due to the autoregressive nature of models. 
We evaluate this in detail in \S~\ref{error}. 


\noindent{\bf Practicality.} Crucially, \auto finds approaches that are {\em general and reusable} across similar reasoning problems. We reused the strategies identified for solving \textsc{AQuA-RAT} and Planning benchmark respectively in the \textsc{MATH} (counting and probability) and Graph Coloring benchmarks. This also reduces the cost of repeated evaluation on a separate evaluation set.


\noindent{\bf Aggregation.} We aggregate the responses via majority vote for both prompting strategies. Other aggregation strategies can also be leveraged, such as utilizing the LLM itself to aggregate responses or weighted aggregation. In \S~\ref{ss:aggre}, we consider an aggregation strategy proposed by~\citet{yoran2023answering} and describe how compatible it is with our prompting approaches.



==> xkzmfysyngmvcnyzvsrzkvmqbwygckny/latex/content/3_results.tex <==
%\vspace{-2mm}
\section{Results}
\label{sec:results}
\vspace{-2mm}
\subsection{Main Results}

We present the summary of results in Table~\ref{tab:results_1} and ~\ref{tab:results_2}. Detailed results are available in Appendix~\ref{appendix:addiitonal_results}. These also cover results on the impact of ensemble size in Appendix~\ref{appendix:ensemble_size}.


\begin{table}[t]
\centering
\small
\label{tab:comparison_cqa}
\begin{tabular}{cccc}
\toprule
  {\bf Method} & {\bf Graph Coloring} & {\bf BW 3} & {\bf BW 4/5 } \\
\midrule
 CoT  & 15.0 & 70.00   & 40.00\\
  SC-3 & 18.0 & 66.00   & 38.20\\
  SC-5 & 20.0 & 70.00   & 38.40 \\
  SC-7 & 22.0 &72.00   & 40.00 \\
  SC-10 & 23.0 & 73.00    &41.20 \\
      \idivse & 74.00 & 82.00   & 57.00 \\
      \divse & {\bf 97.00} & {\bf 94.00}  &  {\bf 69.60} \\

\bottomrule
\end{tabular}
\caption{Performance on \textsc{Graph Coloring} and  \textsc{Blocksworld} planning for GPT-4 in the ZS-CoT setting. We compare \divse and
\idivse with SC~\citep{wang2023selfconsistency} and CoT~\citep{wei2022chain}.}
\label{tab:results_1}
\end{table}


\begin{table}[ht]
\centering
\small
\label{tab:comparison_cqa}
\begin{tabular}{ccccccc}
\toprule
{\bf Setting} & {\bf Method} & {\bf AQuA} & {\bf MATH}  & {\bf CQA }\\
\midrule
\multirow{5}{*}{GPT-3.5 ZS} & CoT  & 59.00 & 31.90   &  71.40\\
 & SC-3 & 61.40  & 32.07   &  72.00\\
   & SC-5 & 63.37 & 38.19  &   72.80\\
     & \idivse & 62.60 & 42.50   &  74.00\\
     & \divse & {\bf 72.83} & {\bf 44.94}   & {\bf 74.50} \\ \hline
% & &  &   &  & \\
     \multirow{3}{*}{GPT-3.5 FS} & CoT  & 57.48 & 30.38   &  79.4\\
     & \idivse & 64.57 & 44.10 &  80.00  \\
     & \divse & {\bf 72.84} & {\bf 52.22} &  {\bf 80.40}  \\
\midrule
    \multirow{3}{*}{GPT-4 ZS} &  CoT  & 70.47 & 62.24    & 81.60\\
     & \idivse & 71.65 & 72.00   &  {\bf 82.50 }\\
     & \divse & {\bf 80.31} & {\bf 79.11}    & 81.70\\ \hline
    % & &  &   & & \\
  \multirow{3}{*}{GPT-4 FS}  & CoT  & 71.90 & 66.46  & 87.70\\
     & \idivse & 79.90 & 72.00 &  {\bf 89.00 } \\
     & \divse & {\bf 84.25} & {\bf 80.76}   & 88.00\\
\bottomrule
\end{tabular}
\caption{Performance on \textsc{AQuA-RAT}, \textsc{MATH} (Counting and Probability),  and \textsc{CommonsenseQA} for GPT-3.5 Turbo and GPT-4 in the ZS-CoT and few-shot-CoT settings respectively. \vspace{-5mm} 
}
\label{tab:results_2}
\end{table}

\subsubsection{Arithmetic reasoning via \textsc{AQuA-RAT}} 
\noindent{\em GPT-4 Results:} In Table~\ref{tab:results_2}, we observe that \divse achieves an accuracy increase of 9.84 and 14.6 p.p in the FS-CoT (baseline accuracy of 71.9\%) and ZS-CoT (baseline of 70.47\%) settings, respectively. While the gains from \idivse are nominal in ZS-CoT, it achieves a boost of 7.7 p.p for FS-CoT.

\noindent{\em GPT-3.5 Results:} In Table~\ref{tab:results_2}, we see that \divse yields a gain of 14.23 and 16.52 p.p in the FS-CoT (baseline of 57.48\%) and ZS-CoT (baseline of 59\%) settings, respectively. Within the FS-CoT setting, \idivse gets an absolute increase of 7 p.p.

Note that Fig.~\ref{fig:cost_vs_accuracy_plot_mert} also displays the total inference cost. Both \idivse and \divse are {\em Pareto optimal}, indicating their capacity to achieve a higher accuracy while maintaining low costs.

\subsubsection{Counting and probabilistic reasoning via \textsc{MATH}} 


\noindent{\em GPT-4 Results:} From Table~\ref{tab:results_2}, we see that \divse achieves an accuracy increase of 14.3 and 16.87 p.p in the FS-CoT (baseline of  66.46\%) and ZS-CoT (baseline of 62.24\%) settings, respectively. On the other hand, \idivse achieves a boost of 5.54 and 9.76 p.p in the FS-CoT and ZS-CoT settings, respectively, over the baseline.


\noindent{\em GPT-3.5 Results:} From Table~\ref{tab:results_2}, we see that \divse yields a gain of 21.84 and 13.04 p.p in the FS-CoT (baseline of 30.38\%) and ZS-CoT (baseline of 31.90\%) settings, respectively. Likewise \idivse achieves a boost of 13.72 and 10.60 p.p in the FS-CoT and ZS-CoT settings, respectively.


\subsubsection{Planning via \textsc{Blocksworld}}

 \noindent{\em Setup:} The benchmark provides both natural language and Planning Definition and Domain Language prompts~\citep{mcdermott1998pddl}.
 We use natural language prompts in all the experiments. For the baseline runs, we introduce minor alterations to the prompt originally proposed by~\citet{valmeekam2023planning}. These changes involve incorporating an explicit directive to prevent under-block movement and resolving minor language ambiguities we observed to be problematic during initial investigation. Furthermore, we reposition the initial condition and goal state information to the beginning of the prompt. The modified improved prompt is presented in Fig.~\ref{fig:planning_baseline_prompt}. 
 
We aggregate the plans through majority voting and utilize string matching for comparing the plans. As a result, we optimize the plan by eliminating the redundant ``\texttt{no-op}'' steps.

\begin{comment}
\begin{Verbatim}[commandchars=\\\{\}]
\centering
[(unstack b c), (stack a b), (unstack a b), (stack b a)] ==
[(unstack b c), \sout{(stack a b)}, \sout{(unstack a b)}, (stack b a)] 
\end{Verbatim}
\end{comment}


\noindent{\em GPT-4 Results:} We note that GPT-4 performs slightly better in a ZS setting, and use this to run all experiments. From Fig.~\ref{fig:cost_vs_accuracy_plot_mert}, we observe that for \textsc{Blocksworld 3}, ZS-CoT records an accuracy of 70\%, while SC-10 reaches an accuracy level of 73\%. \idivse enhances the absolute accuracy by 12 p.p above the ZS-CoT baseline, while \divse produces an impressive {\em state-of-the-art} accuracy of 94\%. An analysis of the six unsuccessful instances suggests the capacity for further performance improvement by increasing the size of the ensemble, as already two out of five current approaches generate accurate plans. For the \textsc{Blocksworld 4/5} case, the ZS-CoT accuracy is 40\%, while SC-10 has an accuracy of 41.2\%. Here, \idivse results in an absolute gain of 17 p.p above the ZS-CoT baseline, and \divse too enhances performance, leading to 69.6\%. As outlined in Fig.~\ref{fig:cost_vs_accuracy_plot_mert} and ~\ref{fig:cost_vs_accuracy_plot_mert2}, both \idivse and \divse achieve {\em Pareto optimality}. 

\noindent{\em GPT-3.5 Results:} The baseline performance on \textsc{Blocksworld 3} is 6\%, and on \textsc{Blocksworld 4/5} is 0.6\%. We do not see any additional improvement using both \idivse and \divse. Qualitatively, we observe that during plan generation, GPT-3.5 fails to follow the restrictions provided as part of the problem instructions too often, leading to either infeasible or incorrect plans. This shows instruction following capabilities are crucial to the success of the methods proposed here.

\subsubsection{Constraint Satisfaction via \textsc{graph Coloring}}
There may exist numerous non-optimal yet valid colorings for a given graph. Since exact string matching is not usable for identifying the majority solution from the ensembles of \idivse and \divse, we employ the external, sound verifier~\citep{stechly2023gpt4} to pick the correct solution.

\noindent{\em GPT-4 Results:} From Fig.~\ref{fig:cost_vs_accuracy_plot_mert}, it is observed that ZS-CoT achieves an accuracy of 15\%, whereas SC-10 attains an accuracy level of 23\%. \idivse improves the absolute accuracy by 59 p.p above the ZS-CoT baseline. Remarkably, \divse delivers a {\em state-of-the-art} accuracy of 97\%. Given that GPT-4's performance plateaus in the ZS setting, we  chose to omit conducting the few-shot experiments.


\noindent{\bf Summary:} Methods in this work often demonstrate state-of-the-art performance on reasoning tasks. This is most significant in the planning and constraint satisfaction benchmarks, where the corresponding authors claimed immense difficulty for existing LLMs. Our work shows that status-quo prompt design approaches including chain of thought are too generic for these problems, and prompt customization (via \auto) can yield substantial gains by guiding the chain of thought to the general nature of the problem.



\subsection{Open Source Models}

Due to the limited computational budget, we only performed experiments with the \textsc{AQuA-RAT} benchmark. Please refer to Appendix~\ref{appendix:open-source} for further details. Table~\ref{tab:open-source} demonstrates the results for LLaMA-2 70B with 8-bit quantization. \divse and \idivse demonstrate an improvement of over 10 p.p over the baseline in the FS-CoT settings. However, the gain in the ZS-CoT setting has been negligible. We hypothesize that this is partly due to model's lack of capabilities to both follow instructions and the mentioned approach in the absence of examples. 

\begin{table}[!ht]
  \centering
    \small
  \label{tab:comparison_prompting_strategy}
  \begin{tabular}{lcc}
    \toprule
     {\bf Prompting Strategy} & {\bf ZS-CoT (\%)} & {\bf FS-CoT (\%)} \\
    \midrule
    CoT & 31.32 & 29.1 \\
    \idivse & 27.00 & 39.7 \\
    \divse & \bf{32.00} & \bf{39.9} \\

    \bottomrule
  \end{tabular}
      \caption{Results on \textsc{AQuA-RAT} and LLaMA-2 70B.\vspace{-5mm}}
      \label{tab:open-source}
\end{table}


\subsection{Errors \& Prompt Utility} 
\label{error}


\noindent{\em Error Propagation:} Due to the autoregressive nature of LLM decoding, early incorrect answers in \idivse may get propagated to the latter ones. To quantify this, we select examples where the solution is incorrect and all five approaches produce the same erroneous answer. We focus only on these cases to see if e.g., a wrong conclusion in the initial approaches leaks into the following ones. Next, we attempt the last two approaches again in a separate session: if the LLM generates the same outcomes as in the original session (i.e., \idivse setup) within 3 attempts, we consider it as no error propagation. However, if it does not produce the same answer within the 3 attempts, we interpret this as a case of error propagation since the change in answer could be attributed to the initial approaches with wrong answers in the chain. We measure this phenomenon on \textsc{AQuA-RAT} (FS-CoT) on both GPT-4 and GPT-3.5. We find that GPT-4 and GPT-3.5 have error propagation rates of 6.2\% and 5.5\% respectively, which are comparable to performance differences between \divse and \idivse, {\em making error propagation one of the main explanatory hypotheses for the differences between the two methods}. Reducing these error rates remains a challenging problem given the autoregressive nature of current LLMs. 


\begin{table*}[!ht]
  \centering
\small
  \begin{tabular}{cll}
\toprule
    {\bf Dataset, Model} & {\bf Persona, Approach} & {\bf Accuracy (\%)}  \\
\midrule
    \multirow{3}{*}{\textsc{AQuA-RAT}, GPT-3.5} & $\emptyset$,Think step by step & 57.48  \\
    & $\emptyset$, Using Algebra & 60.24 \footnotesize{\bf (+2.76)} \\
    & Thinking like Alan Turing, $\emptyset$ & 61.81 \footnotesize{\bf (+4.33)}  \\
        & Dr. Patel: A renowned mathematician, $\emptyset$ & {\bf 65.75 \footnotesize{(+8.27)}}  \\
    \hline
    \multirow{3}{*}{\textsc{Blocksworld 4/5}, GPT-4} & $\emptyset$, State tracking prompt~\citep{valmeekam2022large} & 42.00  \\
    & \textcolor{blue}{$\emptyset$, Finite State Machine} & 55.80 \footnotesize{\bf (+13.80)} \\
    & \textcolor{blue}{Alan Turing, Action Rationale} & 57.80 \footnotesize{\bf (+15.80)}  \\
  & \textcolor{blue}{Alan Turing, Progressive Block Placement Approach} & {\bf 58.80 \footnotesize{(+16.80)}}  \\
\bottomrule
  \end{tabular}
    \caption{\textbf{Prompts, derived from approaches and personas, boost performance.} \textcolor{blue}{Blue} rows denote ZS-CoT prompts, while black lines denote FS-CoT prompts. $\emptyset$ denotes absence (of persona or approach respectively). 
    }
 \label{fig:personas_approaches}
\end{table*}

\noindent{\em Beyond Thinking Step by Step:} The diverse approaches and personas we utilize not only enhance the performance in \idivse and \idivse, but are also independently superior to ZS-CoT. Table~\ref{fig:personas_approaches} highlights this effect, which showcases the importance of conditioning the model for solutions via \auto.

\subsection{Alternative Aggregation Strategies}
\label{ss:aggre}

\begin{table}[t]
  \centering
    \small
  \label{tab:comparison_agg_strategy}
  \begin{tabular}{lcc}
    \toprule
     {\bf Method} & {\bf GPT-4 (\%)} & {\bf GPT-3.5 (\%)} \\
    \midrule
    Majority Voting & {\bf 79.90} & 64.47 \\
    Meta Reasoning & {79.24} & {\bf 67.70} \\
    \bottomrule
  \end{tabular}
      \caption{{\bf Alternative aggregation strategies.} Observe that, for the \textsc{AQuA-RAT} benchmark (FS-CoT), \idivse produces more accurate results only with GPT-3.5. \vspace{-5mm}}
      \label{tab:meta}
\end{table}

Our aggregation thus far relies on majority voting. Alternatively, we can also utilize the meta reasoning technique proposed by~\citet{yoran2023answering} to accumulate the results and exploit the rich information present in the reasoning steps.
To this end, we store the responses generated by \idivse, and request the model to meta reason over them in a different prompt and session. Table~\ref{tab:meta} suggests that the proposed reasoning paths contain rich information that is effectively exploited by the meta reasoning aggregation. Future post-hoc  techniques may consider to learn the accuracy of the diverse prompting approaches, and weigh them accordingly. Nevertheless, the fact that techniques presented here provide visible improvements even with simple approaches like majority voting, demonstrates their added value independently from different aggregation algorithms. 



==> xkzmfysyngmvcnyzvsrzkvmqbwygckny/latex/content/4_related_work.tex <==
\section{Related Work}
\label{sec:related}
\noindent{\bf Prompt Optimization:} \citet{pryzant2023automatic} models the prompts as optimizable discrete variables, and minimizes the loss of the reasoning task. \citet{jones2023automatically} optimize over the prompt space, but to identify failure modes. However, optimization-based approaches often require the task to have a differentiable loss function, which is a strong condition. In our work, we utilize feedback from the LLM (not through gradients) during prompt design. Similarly to~\citet{cheng2023batch}, \idivse batches the responses for multiple queries within a prompt.

\noindent{\bf Decoding Optimizations and Tools:}~\citet{wang2023selfconsistency} replace the naive greedy decoding by sampling a diverse set of reasoning paths (e.g., through temperature sampling), and then selects the most consistent answer. ~\citet{chen2022program} express the reasoning process as a program, which is then delegated to an external tool. 
In our work, we neither change the decoding process nor assume the existence of trusted tools. This makes our solution directly applicable to black-box models.

\noindent{\bf Prompting Strategies:} ~\citet{brown2020language} note that demonstrations to prompts, encoded as input-output pairs, produce drastic performance increase in larger LLMs.~\citet{wei2022chain} encourage internal dialogue by forcing the LLM to generate a sequence of intermediate steps for reasoning problems. This improves reasoning performance on larger LLMs~\citep{nye2021show,chung2022scaling, kojima2022large}. ~\citet{zhou2022least} automatically break a complex problem into simpler sub-problems and then solve them in sequence. Across all these techniques, the common practice is to keep the prompts fixed, but aggregate responses across multiple trials by varying the temperature. In our work, we vary the input prompt itself. A work that is similar in spirit is that of~\citet{yoran2023answering}, which instead of aggregating the response of multiple reasoning paths, forces the model to reason across them before aggregation. Another relevant work is that of \citet{li2023making}, which shows the importance of prompt diversity. However, they rely on selecting few-shot demonstrations from a hold-out set (which defines diversity in their method), without explicitly stating reasoning pathways. 



==> xkzmfysyngmvcnyzvsrzkvmqbwygckny/latex/content/5_conclusions.tex <==
\section{Conclusions}
In this work, we promoted diversity of thought as a principled prompting strategy and proposed methodologies that leverage the LLM as a guide to design a diverse set of approaches to solve complex reasoning tasks. Extracting solution approaches from LLMs themselves becomes a discovery mechanism that seeds and conditions generative solutions. 
Reported results on a variety of tasks confirm that there is a large space for improvement in complex reasoning by uncovering the necessary skills and knowledge from LLMs through targeted and diverse prompting methods. These results demonstrated how promoting diversity can improve the Pareto frontier of accuracy-cost trade-off for current LLMs and yield {\em state-of-the-art} solutions for planning and mathematical reasoning tasks. We hope that future work will expand these results to complex tasks from other real-world applications. 


\section{Limitations}
Our study mainly experimented with GPT-3.5 and GPT-4 models because of their instruction-following capabilities. While current open-source models have shown remarkable improvements to this end, they are still not able to reliably follow instructions relevant to complex reasoning tasks (e.g. state tracking, plan validity, constraint satisfaction). We hope that progress in the field will enable further experimentation in this direction. 

In addition, we also observe that error propagation during autoregressive generation may sometimes negatively impact the performance of \idivse, where all approaches are executed in order within the same prompt. Some of this could be addressed by explicitly instructing the model to forget about the previous solution but ultimately as long as previous generation history remains in context and short-term memory, error propagation risks may still need to be tracked and measured. 






==> xkzmfysyngmvcnyzvsrzkvmqbwygckny/latex/content/algorithm.tex <==

\begin{algorithm}[t]
\footnotesize
\captionsetup{labelformat=empty}
\caption{{\em \auto}: Prompt creation.}
\begin{algorithmic}
\Procedure{DiversePrompt}{\texttt{size, type}, $F, D, V$}
\State \LeftComment \textbf{Step 1: Identify different approaches to be used.}
\State $A = \{a_1, \ldots, a_{n}\} \gets \texttt{det\_approaches}(\texttt{D})$ 
\LeftComment{where $A$ is the set of approaches}
\State \LeftComment \textbf{Step 2: Identify different personas to be used.}
\State $P = \{\phi, p_1, \ldots, p_{m}\} \gets \texttt{det\_personas}(\texttt{D})$ 
\LeftComment{where $P$ is the set of personas}
\State \LeftComment \textbf{Step 3: Find the best combination.}
%of approaches and personas.}
\State $ S = \{s_1, \ldots\, s_{\texttt{size}}\} \gets \texttt{combine}(A, P, \texttt{size}, V)$ 
\LeftComment{where $S$ is the set of combined approaches and personas, and $s_i = (p, a_{i} \in A)$}
\State \LeftComment \textbf{Step 4: Augment the few-shot examples.}
%\State $T = \{f((p_i, a_j), FS), f((p_i, a_k),_FS),\ldots\} \gets \texttt{transfer}(S, F)$ \LeftComment{where $T$ is the set of style-transferred examples}
\State $T = \{\tilde{T}_{i,j}, \ldots\} \gets \texttt{augment}(S, F)$ \LeftComment{where $T$ is the set of augmented examples, and $\tilde{T}_{i,j}$ is formed using $s_i \in S$ and $f_j \in F$; $|T|=$\texttt{size}}
\State \LeftComment \textbf{Step 5: Compose the final prompt.}
%based on $T$, $S$, and \texttt{type}.}
\State $O \gets \texttt{compose}(T, S, \texttt{type})$ 
\State \textbf{return } $O$ \LeftComment{Return the final output.}
\EndProcedure
\end{algorithmic}
\label{alg_1}
\end{algorithm}






==> xkzmfysyngmvcnyzvsrzkvmqbwygckny/latex/content/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
%\noindent{\bf Tasks \& Datasets.} 
We consider the following reasoning benchmarks.
%\begin{enumerate}[leftmargin=*,itemsep=0.0ex, parsep=0pt] 

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{latex/figures/cost_vs_accuracy_gsm_cqa_besa_feedback.pdf}
    \caption{\textbf{Diversity of Thought enhances the inference cost and accuracy trade-off.} We compare \divse and \idivse with SC~\citep{wang2023selfconsistency} and CoT~\citep{wei2022chain} across three benchmarks. The x-axis indicates the total cost (as defined in \S~\ref{sec:experiments}) of running inference with the LLM on the benchmark using the given method, while the y-axis represents the LLM’s performance. The FS-CoT setting is represented by filled gray dots, while the ZS-CoT setting is indicated by unfilled dots. Notice that for \textsc{Blocksworld 3}, despite being in the ZS-CoT setting, our approaches are more performant than the SC-$s$ (FS-CoT) baseline.\vspace{-5mm}}
    \label{fig:cost_vs_accuracy_plot_mert2}
\end{figure*}


\noindent {\em Arithmetic Reasoning}:  We use: (i) \textsc{AQuA-RAT}~\citep{ling-etal-2017-program}, a suite of algebraic word problems,  (ii) \textsc{GSM8K}~\citep{cobbe2021training}, a benchmark of grade-school math problems described in natural language (involving elementary arithmetic operations), and (iii) \textsc{MATH} (Counting and Probability)~\citep{hendrycks2021measuring}, a collection of math problems from which we choose only counting and probability as these are not covered by \textsc{GSM8K} and \textsc{AQuA-RAT}. For all datasets, we use the \texttt{test} split for evaluation, containing 254, 1319, and 474 questions respectively. 

\noindent {\em Planning Capabilities}: We use the Blocksworld Planning benchmark proposed in \citet{valmeekam2022large, valmeekam2023planning}. 
The benchmark has two datasets: one involves 3 blocks (\textsc{Blocksworld 3}, 100 instances), while the other dataset involves 4 or 5 blocks (\textsc{Blocksworld 4/5}, 500 instances). 

\noindent {\em Constraint Satisfaction Optimization}: We use the \textsc{Graph coloring} benchmark~\citep{stechly2023gpt4} containing 100 examples to test reasoning for constraint satisfaction.

\noindent {\em Commonsense Reasoning}: We use \textsc{CommonsenseQA}~\citep{talmor-etal-2019-commonsenseqa} which consists of generic multiple-choice questions elicited for testing common sense reasoning. We use the \texttt{validation} split containing 1,221 questions.


\noindent{\bf Language Models.} We evaluate our proposed methods on both GPT-3.5 Turbo~\citep{chatgpt} and GPT-4~\citep{gpt4}. We also conduct an additional evaluation on LLaMA-2 70B~\citep{touvron2023llama2} to explore the performance of our technique on open-source LLMs. For the latter, we use \texttt{meta-llama/Llama-2-70b-chat-hf} through the Transformers library~\citep{wolf2019huggingface}.



\noindent{\bf Baselines.} We consider Chain-of-Thought (CoT)~\citep{wei2022chain} and Self-Consistency (SC~)~\citep{wang2023selfconsistency} as our baselines. For CoT, we consider two settings: zero-shot (ZS) CoT~\citep{kojima2022large} (i.e., ``\texttt{Think step by step}'' is added to the prompt), and few-shot (FS) CoT (i.e., CoT with demonstrations). In our SC runs, we set the temperature $T=0.7$ without top-$k$ truncation and sample up to $s \in [1,10]$ outputs (denoted SC-$s$). For all other approaches, we set $T=0$. We use ensembles of size 5 in \idivse and  \divse for \textsc{GSM8K} and \textsc{AQuA-RAT}. For the planning, \textsc{Graph Coloring}, and \textsc{CommonsenseQA} benchmarks, we use a size of 3. 

%\iffalse
\noindent{\bf Performance Metrics.} We measure the accuracy on the task, and the generation inference cost.To measure the cost, we assume 1000 tokens are about 750 words\footnote{https://openai.com/pricing}. For GPT-4 (8K) the input and output prices used to estimate inference cost are \$0.03/1k tokens and \$0.06/1k tokens, respectively. For GPT 3.5 Turbo (16K), the input and output prices used in the cost estimation are \$0.003/1k (tokens) and \$0.004/1k (tokens) respectively. 
%\fi

\noindent{\bf Results Summary.} %Salient features of our results include:
\noindent 
\noindent Across most benchmarks we consider, our techniques provide substantial performance gains (e.g., 16.52, 82.5, and 14.3 p.p improvements for \textsc{AQuA-RAT}, \textsc{Graph Coloring}, and \textsc{MATH} respectively). They are also Pareto optimal (in terms of the utility vs. cost trade-off). For the challenging planning benchmark (\textsc{Blocksworld 4/5}), our techniques improve accuracy by 29.6 p.p achieving {\em state-of-the-art} performance. Using GPT-4 for \textsc{Blocksworld 3}, our approach (in the ZS-CoT setting) is substantially more effective than SC-10 (in the FS-CoT setting) at 4$\times$ lower cost (Figure~\ref{fig:cost_vs_accuracy_plot_mert2} (center figure)). 

Since prompts are chained together in \idivse, error propagation is possible. Our evaluation on \textsc{AQuA-RAT} in ~\S~\ref{error} suggests that even though error propagation is estimated as less than 6.5\% for both models, these rates are comparable to differences in performance between \divse and \idivse. 
\noindent When combined with aggregation approaches that are capable of reasoning across the diverse generations~\citep{yoran2023answering}, we observe additional performance gains as shown in ~\S~\ref{ss:aggre}. For the \textsc{AQuA-RAT} benchmark for instance, we see an accuracy of 67.7\% for GPT-3.5 (3.23 p.p improvement to majority voting). 
%\end{enumerate}

==> xkzmfysyngmvcnyzvsrzkvmqbwygckny/latex/figures/intro_fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{latex/figures/cost_vs_accuracy_v2.pdf}
    \caption{\textbf{Diversity of Thought enhances the inference cost and accuracy trade-off.} We compare \divse and \idivse with SC~\citep{wang2023selfconsistency} and CoT~\citep{wei2022chain} across three benchmarks. Panels show (i) AQUA-RAT on GPT-3.5 in few-shot-CoT setting, and (ii) Blocksworld 3 and 4/5 on GPT-4 in zero-shot-CoT setting. The x-axis indicates the total cost (as defined in \S~\ref{sec:results}) of running inference with the LLM on the benchmark with the given approach, the y-axis indicates the LLM's performance, and the color indicates the approach (and whether it is zero-shot-CoT or few-shot-CoT).}
    \label{fig:cost_vs_accuracy_plot_mert}
\end{figure}




==> xkzmfysyngmvcnyzvsrzkvmqbwygckny/latex/figures/prompt_example.tex <==
\definecolor{lightgray}{RGB}{240,240,240} %
\renewcommand{\sfdefault}{cmss} % Computer Modern Sans Serif
\begin{figure*}[!th]
\begin{tcolorbox}[
    enhanced,
    opacityback=0.2,
    opacityframe=0.2,
    colback=lightgray,
    colframe=lightgray, 
    top=1mm, 
    bottom=1mm, 
    left=1mm, 
    right=1mm,
    %sharp corners,
    fontupper=\sffamily\small,
    ]    
\begin{small}
\noindent

Use five distinct approaches to solve the given problem accurately. If there is no exact match choose the closest option.

Q: \{Question\}

Use the following output format:

Approach 1 {< name of the approach >} : {< Details of Approach 1} >

Approach 2 {< name of the approach >} : {< Details of Approach 2} >

Approach 3 {< name of the approach >} : {< Details of Approach 3} >

Approach 4 {< name of the approach >} : {< Details of Approach 4} >

Approach 5 {< name of the approach >} : {< Details of Approach 5} >
\noindent
\end{small}
\end{tcolorbox}
\caption{Prompt template for extracting diverse approaches for problem solving.}
\label{fig:auto-example}
\end{figure*}

\clearpage

==> xkzmfysyngmvcnyzvsrzkvmqbwygckny/latex/figures/system_fig.tex <==
\begin{figure*}[t]
\centering
\begin{minipage}[t]{0.9\textwidth}
\includegraphics[width=\linewidth]{latex/figures/system_diagram_1_3.pdf}
\end{minipage}
\caption{\textbf{Diversity of Thought}. This illustration depicts CoT and \idivse prompting strategies. Notice that both have a single example. However, \idivse presents more diversity in terms of reasoning paths. This enables it to generate diverse completions, yielding more accurate responses.\vspace{-5mm}}
\label{fig:overall}
\end{figure*}


